Robust Snapshot Radio SLAM

The intrinsic geometric connections between millimeter-wave (mmWave) signals and the propagation environment can be leveraged for simultaneous localization and mapping (SLAM) in 5G and beyond networks. However, estimated channel parameters that are mismatched to the utilized geometric model can cause the SLAM solution to degrade. In this paper, we propose a robust snapshot radio SLAM algorithm for mixed line-of-sight (LoS) and non-line-of-sight (NLoS) environments that can estimate the unknown user equipment (UE) state, map of the environment as well as the presence of the LoS path. The proposed method can accurately detect outliers and the LoS path, enabling robust estimation in both LoS and NLoS conditions. The proposed method is validated using 60 GHz experimental data, indicating superior performance compared to the state-of-the-art.

==> results_old.tex <==
\section{Experimental Results}\label{sec:results}

\begin{figure*}
\centerline{
\subfigure[Example solution]{\includegraphics[trim={1cm 0.1cm 2.2cm 0.8cm]},clip=true,width=6cm]{figures/SLAM_example.pdf}
\label{fig:SLAM_example}}
\hfil
\subfigure[Proposed method]{\includegraphics[trim={1cm 0.1cm 2.2cm 0.8cm]},clip=true,width=6cm]{figures/SLAM_performance.pdf}
\label{fig:SLAM_performance}}
\hfil
\subfigure[Benchmark method w/o outliers]{\includegraphics[trim={1cm 0.1cm 2.2cm 0.8cm]},clip=true,width=6cm]{figures/SLAM_performance_benchmark.pdf}
\label{fig:SLAM_performance_benchmark}}
}
\caption{Example SLAM performance using the proposed and benchmark methods. In (a), the obtained snapshot SLAM solution using the proposed method in one measurement position. In the figure, the TX and RX locations illustrated with (\protect\bluetriangle), RX position estimate with (\protect\redtriangle), LoS path using (\protect\redline), single-bounce NLoS paths with solid lines, propagation paths that are identified as outliers shown using dashed lines (plotted by plugging $\gamma_i = 0.5$ in to the single-bounce model in \eqref{eq:rx_position}) and the dotted ellipses illustrate the two standard deviation uncertainty ellipse of the RX and landmark position estimates. In (b) and (c), the RX and landmark position estimates for all $45$ measurement positions. The legend of the figures is: TX location (\protect\bluetriangle), ground truth RX positions (\protect\blueline), RX position estimates (\protect\blackcross) and landmark estimates (\protect\redplus). Landmark estimates around coordinate $\hat{\vp}_i = [9.4, \; 0.8]^\top$ and that appear inside a room result from a triple-bounce reflection for which the incidence points are on the two walls beside the TX. This propagation path is inline with the single-bounce model and therefore it is not classified as an outlier.}
\label{fig:experimental_results}
\end{figure*}

\subsection{Experimental Setup}

The indoor measurement campaign has been carried at Tampere University campus using two Sivers Semiconductors Evaluation Kit EVK06002 \cite{EVKinfo} as TX and RX. The setup was emulating downlink (DL) communication case with a stationary TX EVK representing base station (BS) and a quasi-mobile RX EVK representing user equipment (UE). All together, $45$ UE locations were measured. Measurements were carried out at central frequency of $60$~GHz with $400$~MHz band using 5G NR-specified Positioning Reference Signal (PRS) for sensing. Pre-recorded TX waveform for each TX beam has been sent to the EVK via PC-controlled  arbitrary waveform generator M8195A, while Keysight DSOS804A oscilloscope has been used as receiver. PRS was beamformed using Sivers original $63$-beam beambook so that each TX beam is assigned a unique PRS identity number (PRS ID). Since beamforming field of view (FOV) of the EVK antenna array is $[-45^{\circ},45^{\circ}]$, TX and RX EVKs were rotated using FLIR Pan Tilt PTU-46 to cover $180^{\circ}$ in transmission and $360^{\circ}$ in reception. PRS identities $[0:62]$ were used repeatedly for each $90^{\circ}$ window defined by the analog beamforming. Exhaustive beam search was performed to obtain data from all TX-RX beam pair combinations. The details of the experimental setup, used hardware and channel estimator are further discussed in \cite{rastorguevafoi2023}. 

The proposed \ac{SLAM} algorithm utilizes the following parameters in the evaluations. In \ac{NLOS} scenarios, \eqref{eq:robust_cost} is solved with $1^\circ$ angle resolution ($\lvert \mathcal{A} \rvert = 360$). We utilize parameters of the generic $60$ GHz path loss model (see \cite[Table III]{smulders2009}): $\zeta = 1.7$ and $\sigma = 1.8 \text{ dB}$, and $L_0 = 13 \text{ dB}$ is calibrated from data. The \ac{LOS} detection threshold in \eqref{eq:los_detector} is $T = -10$ and the inlier detection threshold used in Algorithm \ref{alg:robust_SLAM_algorithm} is $\varepsilon = 1$. 

\subsection{Results}

\subsubsection{Qualitative Comparison}

 The \ac{SLAM} solution in one example measurement position is illustrated in Fig.~\ref{fig:SLAM_example} using the proposed method. In the example, the proposed method can correctly resolve the \ac{LOS} and single-bounce \ac{NLOS} paths leading to an accurate \ac{SLAM} solution in which the RX position estimate is close to the ground truth and the landmark position estimates closely align with the floor plan of the experimental environment. As illustrated in the figure, the propagation paths that are identified as outliers correspond to three double-bounce propagation paths and one triple-bounce propagation path (dashed green line). In all $45$ measurements positions, the proposed method can accurately identify the propagation paths that are inline with model in \eqref{eq:rx_position} leading to good \ac{SLAM} performance as illustrated in Fig.~\ref{fig:SLAM_performance}. Since the benchmark method cannot inherently deal with outliers, they are removed from the data. The \ac{SLAM} performance for the benchmark method is illustrated in Fig.~\ref{fig:SLAM_performance_benchmark} and as shown, the method is clearly not as accurate even though the outliers have been removed. 
 
 \subsubsection{Quantitative Comparison}

\begin{table}[!t]
\renewcommand{\arraystretch}{1.1}
\caption{RMSE of the proposed and benchmark methods. CPU time is reported using both Matlab MEX / m-file implementations.}
\vspace{-.2cm}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Method & Pos. [m] & Head. [deg] & Clk. [ns] & Time [ms]  \\  \hline
Proposed  & $0.43$ & $2.39$ & $1.64$ & $2.94 \; / \; 142.63$ \\ 
Benchmark  & $11.12$ & $83.79$ & $46.52$ & $0.93 \; / \; 24.35$ \\ \hline
Proposed$^\star$ & $0.41$ & $2.20$ & $1.61$ & $0.53 \; / \; 24.18$ \\ 
Benchmark$^\star$ & $1.46$ & $4.55$ & $4.97$ & $0.77 \; / \; 19.79$ \\\hline
Proposed$^\dagger$ & $0.32$ & $1.95$ & $1.23$ & $0.02 \; / \; 0.33$ \\ 
Proposed$^\ddagger$ & $0.61$ & $3.23$ & $2.35$ & $10.11 \; / \; 492.84$ \\ \hline
\multicolumn{5}{l}{$^\star$outliers removed from data; $^\dagger$LoS scenario; $^\ddagger$NLoS scenario.} \\
%\multicolumn{5}{l}{$^\star$outliers removed from data; $^\dagger$only LOS scenario, $32/45$ measurement} \\
%\multicolumn{5}{l}{positions; $^\ddagger$only NLOS scenario, $13/45$ measurement positions.} \\
\end{tabular}
\label{table:performance_summary}
\vspace{-.0cm}
\end{table}

Since the ground truth landmark locations are unknown, which is a common problem in \ac{SLAM} when using experimental data, the quantitative evaluation focuses on the \ac{UE} state. The position, heading and clock bias \acp{RMSE} are tabulated in Table~\ref{table:performance_summary}, and the performance is summarized both with and without outliers. When the outliers are not removed from the data, the benchmark method yields insufficient performance and the accuracy improves notably when the outliers are removed. The proposed method yields good \ac{SLAM} accuracy in both cases and the results demonstrate that the presented outlier removal method is effective in practice. In the last two rows of Table~\ref{table:performance_summary}, the \acp{RMSE} are reported separately in the \ac{LOS} scenario ($32/45$) and \ac{NLOS} scenario ($13/45$), and as expected, higher accuracy is achieved when the \ac{LOS} is available. 

 \subsubsection{LoS Detection Accuracy}

 In the considered experimental setting, the \ac{LOS} detection routine presented in Section \ref{sec:unknown_los_scenario} yields perfect detection accuracy, $P(\mathcal{H}_0 \mid \text{LoS}) = 1$ and $P(\mathcal{H}_1 \mid \text{NLoS}) = 1$, but it is to be noted that perfect accuracy is not mandatory. To further investigate \ac{SLAM} performance with an imperfect \ac{LOS} detector, we synthetically vary the probability of \ac{LOS} detection, $P(\text{LoS}) \in [0, \, 1]$, and perform $1000$ \ac{MCS} with each value. The result is illustrated in Fig.~\ref{fig:sensitivity_analysis}. Interestingly when $P(\text{LoS}) = 0$, the problem is solved assuming \ac{NLOS} only and the estimated trajectory and map are very similar to the ones presented in Fig.~\ref{fig:SLAM_performance_benchmark}. The position \ac{RMSE} is $1.43 \text{ m}$ and the accuracy is comparative to the benchmark method without outliers, indicating the method is robust to outliers even without the \ac{LOS} detector. Furthermore, as $P(\text{LoS})$ increases, the \ac{RMSE} decreases which suggests that it is beneficial to solve the problem using the \ac{LOS} if it exists. 
 
 Let us further elaborate the difference in solving the problem using the \ac{LOS} or assuming \ac{NLOS}. First of all, one \ac{LOS} measurement position at $\vp = [3.56, \, -5.70]^\top$ is very inaccurate if the \ac{LOS} is misdetected inflating the position \ac{RMSE} shown in Fig.~\ref{fig:sensitivity_analysis}. A significant decrease in \ac{RMSE} is observed if the \ac{RMSE} is computed without the unfavorable position. Without $\vp = [3.56, \, -5.70]^\top$, the \ac{RMSE} is $0.57 \text{ m}$ when $P(\text{LoS})=0$ and it decreases down to $0.43 \text{ m}$ as the probability of \ac{LOS} detection increases to $P(\text{LoS})=1$. This performance improvement is more apparent observing the median of the position error \acp{CDF} illustrated in Fig.~\ref{fig:sensitivity_analysis}. The \ac{CDF} of $P(\text{LoS}) = 0$ also clearly shows the heavy-tailed error distribution caused by the unfavorable position. Now the main benefit of exploiting the \ac{LOS} is that the angles define the entire geometry up to a scaling since the \ac{UE} orientation is solved in closed-form and the scaling is determined by the clock bias. In addition, the number of degrees of freedom is lower. Thus, the \ac{SLAM} problem is easier to solve and identifiability of the model is improved leading to increased robustness and enhanced \ac{SLAM} performance when constraints imposed by the \ac{LOS} are exploited.
 

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth,trim={0.0cm 0 0.0cm 0.0cm},clip]{figures/sensitivity_analysis.pdf}%
\caption{On the above, position RMSE as a function of $P(\text{LoS})$ and the legend is defined as: RMSE for all $45$ measurement positions (\protect\blacksquareline); RMSE computed without $\vp = [3.56, \, -5.70]^\top$ (\protect\redtriangleline). In the figure below, position error CDFs with $P(\text{LoS})=0$ (\protect\bluesquareline) and $P(\text{LoS})=1$ (\protect\orangetriangleline).}
\label{fig:sensitivity_analysis}
\end{figure}

 % as shown, the \ac{RMSE} decreases as detection accuracy improves. Interestingly when $P(\mathcal{H}_0 \mid \text{LOS exists}) = 0 \%$, the problem is solved assuming \ac{NLOS} only and the accuracy is comparative to results of the benchmark method without outliers. 
 
 
 % investigate sensitivity of the proposed meth
 % However, further investigation of the proposed \ac{LOS} detector is left for future work since the experimental setting is quite homogeneous and \ac{LOS}/\ac{NLOS} classification is not the main theme of the paper.
 
 % In many of the measurement positions and especially in \ac{NLOS} scenarios, the two methods yield comparative performance. The most notable differences is observed at measurement positions in which the \ac{LOS} exists. At these positions, the proposed method solves the \ac{SLAM} problem exploiting the \ac{LOS}, whereas the benchmark method always assumes an \ac{NLOS} scenario and the constraints imposed by the \ac{LOS} are not exploited. 
 % %Examining the cost in \eqref{eq:cost_function} for the benchmark method reveals that it has multiple local minima and the solution is not always the one that is closest to the ground truth. 
 % It is important to note that utilizing the \ac{LOS} path, the angles determine the entire geometry up to scaling (determined by the clock bias) and the degree of freedom is lower. Thus, the \ac{SLAM} problem is easier to solve and identifiability of the model is improved leading to enhanced \ac{SLAM} performance in several \ac{LOS} measurement positions as illustrated in Fig.~\ref{fig:experimental_results}.

  \subsubsection{Computational Complexity}
  
The computational complexity of the algorithms are given in the last column of Table~\ref{table:performance_summary}, obtained using a Lenovo ThinkPad P1 Gen 2 with a 2.6 GHz Intel i7-9850H CPU and 64 GB of memory. A naive implementation of the proposed and benchmark algorithms scale according to $\mathcal{O}(\lvert \mathcal{A} \rvert \times C)$ and $\mathcal{O}(\lvert \mathcal{A} \rvert)$, respectively. Solving the \ac{SLAM} problem in \ac{LOS} scenarios using the proposed method is very efficient since $\lvert \mathcal{A} \rvert = 1$ and $C = \lvert \mathcal{Z} \rvert - 1$. On the other hand, solving the problem is up to three orders of magnitude higher in \ac{NLOS} scenarios since $\lvert \mathcal{A} \rvert = 361$ and typically $C$ is much larger. With respect to the benchmark method, the computational complexity of the proposed method is lower/higher in \ac{LOS}/\ac{NLOS} scenario and real-time operation with both methods can be easily guaranteed using for example a Matlab MEX-implementations as tabulated in Table~\ref{table:performance_summary}.

